Hybrid static/dynamic scheduling for already optimized dense matrix factorization

We present the use of a hybrid static/dynamic scheduling strategy of the task dependency graph for direct methods used in dense numerical linear algebra. This strategy provides a balance of data locality, load balance, and low dequeue overhead. We show that the usage of this scheduling in communication avoiding dense factorization leads to significant performance gains. On a 48 core AMD Opteron NUMA machine, our experiments show that we can achieve up to 64% improvement over a version of CALU that uses fully dynamic scheduling, and up to 30% improvement over the version of CALU that uses fully static scheduling. On a 16-core Intel Xeon machine, our hybrid static/dynamic scheduling approach is up to 8% faster than the version of CALU that uses a fully static scheduling or fully dynamic scheduling. Our algorithm leads to speedups over the corresponding routines for computing LU factorization in well known libraries. On the 48 core AMD NUMA machine, our best implementation is up to 110% faster than MKL, while on the 16 core Intel Xeon machine, it is up to 82% faster than MKL. Our approach also shows significant speedups compared with PLASMA on both of these systems.

==> pf_data_locality.tex <==
\subsection{Improving data locality in communication avoiding algorithm}
In this section, we aim at modify the dynamic scheduler used in our prior work on CALU such as to take into account the data locality.
\subsubsection{Bloc locality}
 First we introduce a second queue of tasks that are local to each thread. The scheduler has a global queue of the available tasks and for each task it keeps a list of threads which have recently performed an operation on the bloc associated to this task. By this approach, when a thread accesses a bloc more than one time, if it is not in the L1 cache, it could be found in the L2 cache.

In our approach, the scheduler keeps for each bloc a list of threads which have performed an recent operation on this bloc, and each thread keeps a list of blocs on which he has recently performed an operation. Before searching in a global queue, each thread searches an available task in his local queue. To do a good load balancing of the differents queue, we combine our approach with an approach based on the work stealing that is, when a thread fetch a task on a bloc that he did not have yet in its local queue, it deletes it from the queue of the last thread that performed an operation on this bloc. Deleting operation is also important to avoid an exponential memory complexity, for instance we imagine the worst case where each bloc will appear in the local queue of each threads. 

Data locality approach may give unquestionable results when the initial matrix can be decomposed into independant pieces and scheduled to thread without interruption (matrix product for example), this is unfortunately not the case for the LU factorization. After each step, only the panel factorization introduces several tasks in the updating tasks queue. By considering the right looking approach of LU: at each step of the facorization the panel is factorized and then the trailing submatrix are updated column by column from the left to the right. Updating the trailing submatrice from the left is important because it help to make sure that the next panel will be able to start immediatement even if the update of the current step is not complete. However if the next panel start when there are not enough task in the previous step threads will be inactive during the panel factorization. Then any scalable algorithms performing LU factorization must ensure that the panel remains on the critical path. In the dynamic approach with look ahead, threads execute in priority panel tasks as soon as possible to maintain the right execution of the tasks on the critical path however in locality approach they seems executing in priority tasks associated to blocks on which they have recently performed on operation. Therefore, it is trivial to see that the progress of the critical path of the algorithm may be abandoned to preserve the data locality. By the same way, the updating step is still performed from the left to the right but only bloc by bloc on non consecutive column. So, introducing the data locality in algorithm using dynamic scheduler is therefore a tricky businness.  

%The panel factorisation is considerated as a priority task and runs without the locality data allowing to maintain the panel on the critical path and make available spots on the next step.
%incv le temps de rechercche de taches
% le proc executent des taches non prioritaires afin de reutiliser les données
%help thread to acced data already in their cache, tradeoff with runtime DAG execution of the critical task
\subsubsection{Guided bloc locality with column searching}
Our approach on bloc locality can resolve several problems related to cache utilization but other problems can occur: threads search tasks in their local queue before searching in the global queue this imply the increase of the dynamic scheduling time, in the worst case it may double the overload of the scheduler. By the same way, insert and delete element in the thread queue have non-negligible cost. We introduce a second approach based on spatial locality that is, when thread search a task in his local queue  it also search available task on the same column before moving to the next entry in the queue. This approach is based on the spatial locality but does not guarantee that the next bloc will already be loaded in its cache, but it has two more advantages: first, time to search tasks with spatial locality is significantly reduced; second, when it perform an operation on a bloc it move on the next bloc only if the column of that bloc is completely updated, thus help keeping the right looking behaviour of the algorithm which is benefics for the critical path.

%les threads executant le panel sont plus lent donc n'ajoute pas beaucoup de taches à leur queue.
